Understanding normalization in contrastive representation learning and out-of-distribution detection

Contrastive representation learning has emerged as an outstanding approach for anomaly detection. In this work, we explore the $\ell_2$-norm of contrastive features and its applications in out-of-distribution detection. We propose a simple method based on contrastive learning, which incorporates out-of-distribution data by discriminating against normal samples in the contrastive layer space. Our approach can be applied flexibly as an outlier exposure (OE) approach, where the out-of-distribution data is a huge collective of random images, or as a fully self-supervised learning approach, where the out-of-distribution data is self-generated by applying distribution-shifting transformations. The ability to incorporate additional out-of-distribution samples enables a feasible solution for datasets where AD methods based on contrastive learning generally underperform, such as aerial images or microscopy images. Furthermore, the high-quality features learned through contrastive learning consistently enhance performance in OE scenarios, even when the available out-of-distribution dataset is not diverse enough. Our extensive experiments demonstrate the superiority of our proposed method under various scenarios, including unimodal and multimodal settings, with various image datasets.

==> understand_normalization-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Since $EX_i = 0$ for $i \geq 2$ and they are jointly normal distribution, we have \begin {align*} \mathbb {E} \frac {X_i}{\sqrt {X_1^2+X_2^2+\ldots +X_n^2}} = 0 ~ \forall i \in \left \lbrace 2, \dots , n \right \rbrace . \end {align*} Hence, \begin {align*} \mathbb {E}\left \langle \frac {\bm {X}}{\lVert \bm {X} \rVert }, \frac {\bm {Y}}{\lVert \bm {Y} \rVert } \right \rangle & = \mathbb {E} \frac {X_1Y_1}{\lVert \bm {X} \rVert \lVert \bm {Y} \rVert } + \sum _{i=2}^{n} \mathbb {E} \frac {X_iY_i}{\lVert \bm {X} \rVert \lVert \bm {Y} \rVert } = \left (\mathbb {E}\left [ \frac {X_1}{\lVert \bm {X} \rVert } \right ]\right )^2 \end {align*} Let denote $U= X_1$, $V = \left (X_2, \ldots , X_n\right )^t$ and $Z = \lVert V \rVert _2^2 = \sum _{i=2}^{n} X_i^2$. The expectation of cosine similarity between two vectors $\bm {X}$ and $\bm {Y}$ becomes \par \begin {align*} \left (\frac {1}{\sigma \sqrt {2\pi }} \int _{-\infty }^{\infty } \frac {u}{\sqrt {u^2+z}}e^{-(u-\mu )^2/2\sigma ^2}du \int _{0}^{\infty } f_Z(z)dz \right )^2, \end {align*} where $f_Z$ are probability density function of $Z$. \par \noindent \begin {enumerate} \item Let $$A = \frac {1}{\sigma \sqrt {2\pi }} \int _{-\infty }^{\infty } \frac {u}{\sqrt {u^2+z}}e^{-(u-\mu )/2\sigma ^2}du \int _{0}^{\infty } f_Z(z)dz.$$ By the change of variable theorem, replacing $u = u + \mu $ give \begin {align*} A = \frac {1}{\sigma \sqrt {2\pi }} \int _{-\infty }^{\infty } \frac {u+\mu }{\sqrt {(u+\mu )^2+z}}e^{-u^2/2\sigma ^2}du \int _{0}^{\infty } f_Z(z)dz \end {align*} Get derivative, $$A'_\mu = \frac {1}{\sigma \sqrt {2\pi }} \int _{-\infty }^{\infty } \frac {z}{\sqrt {\left ((u+\mu )^2+z\right )^3}}e^{-u^2/2\sigma ^2}du \int _{0}^{\infty } f_Z(z)dz > 0$$ \par \item For \eqref {thm:1:1}, using \cref {lemma:1} we have $f(z) = \int _{-\infty }^{\infty } \frac {u}{\sqrt {u^2+z}}e^{-(u-\mu )/2\sigma ^2}du$ is an decreasing function on $\left [0, \infty \right )$, thus $f(z) \leq f(0) ~\forall z \geq 0$. This gives us \begin {align*} A = \frac {1}{\sigma \sqrt {2\pi }} & \int _{-\infty }^{\infty } \frac {u}{\sqrt {u^2+z}}e^{-(u-\mu )^2/2\sigma ^2}du \int _{0}^{\infty } f_Z(z)dz \\ &\leq \left (\frac {1}{\sigma \sqrt {2\pi }} \int _{-\infty }^{\infty } \frac {u}{\lvert u \rvert }e^{-(u-\mu )^2/2\sigma ^2}du\right ) \left ( \int _{0}^{\infty } f_Z(z)dz\right ) \\ & = \frac {1}{\sigma \sqrt {2\pi }} \left ( \int _{0}^{\infty }e^{-(u-\mu )^2/2\sigma ^2}du - \int _{-\infty }^{0}e^{-(u-\mu )/2\sigma ^2}du \right )\\ & = \frac {1}{\sqrt {2\pi }} \left ( \int _{-\mu /\sigma }^{\infty }e^{-u^2/2}du - \int _{-\infty }^{-\mu /\sigma }e^{-u^2/2}du\right ) \\ & = \Phi \left (\frac {\mu }{\sigma }\right ) - \Phi \left (-\frac {\mu }{\sigma }\right ) \end {align*} For \eqref {thm:1:2}, we have $f(z)$ is convex by \cref {lemma:1}. Jensen's inequality gives us \begin {align*} A = \frac {1}{\sigma \sqrt {2\pi }} \mathbb {E}_{Z}f(Z) \geq \frac {1}{\sigma \sqrt {2\pi }}f(\mathbb {E}_Z(Z)). \end {align*} Since $\mathbb {E}Z = \mathbb {E}\left [\sum _{i=2}^{n} X_i^2 \right ]= \sum _{i=2}^{n}\mathbb {E} X_i^2 = \text {tr}\left (\Sigma _V\right ) = \sigma _V^2$, thus \begin {align} \label {thm1:eq2} A &\geq \frac {1}{\sigma \sqrt {2\pi }}\int _{-\infty }^{\infty } \frac {u}{\sqrt {u^2+\sigma _V^2}}e^{-(u-\mu )^2/2\sigma ^2}du \nonumber \\ &= \frac {1}{\sigma \sqrt {2\pi }}\int _{0}^{\infty } \frac {u}{\sqrt {u^2+\sigma _V^2}}\left (e^{-(u-\mu )^2/2\sigma ^2} - e^{-(u+\mu )^2/2\sigma ^2} \right )du \nonumber \\ &> \frac {1}{\sigma \sqrt {2\pi }}\int _{\epsilon \mu }^{\infty } \frac {u}{\sqrt {u^2+\sigma _V^2}}\left (e^{-(u-\mu )^2/2\sigma ^2} - e^{-(u+\mu )^2/2\sigma ^2} \right )du ~\forall \epsilon >0 \nonumber \\ & \geq \frac {1}{\sigma \sqrt {2\pi }} \left (\frac {\epsilon \mu }{\sqrt {(\epsilon \mu )^2 + \sigma _V^2}}\int _{\epsilon \mu }^{\infty } \left (e^{-(u-\mu )^2/2\sigma ^2} - e^{-(u+\mu )^2/2\sigma ^2} \right )du\right )\\ &= \frac {1}{\sqrt {1+\frac {\sigma _V^2}{\epsilon ^2\mu ^2}}} \frac {1}{\sqrt {2\pi }}\left (\int _{(\epsilon -1)\mu /\sigma }^{\infty }e^{-u^2/2}du - \int _{(\epsilon +1)\mu /\sigma }^{\infty }e^{-u^2/2}du\right )\nonumber \\ &= \frac {1}{\sqrt {1+\frac {\sigma _V^2}{\epsilon ^2\mu ^2}}} \left ( \Phi \left (\frac {(1-\epsilon )\mu }{\sigma }\right ) - \Phi \left (-\frac {(1+\epsilon )\mu }{\sigma }\right ) \right ) \nonumber \end {align} The \cref {thm1:eq2} is due to the fact that $\dfrac {u}{\sqrt {u^2+\sigma _V^2}}$ is an increasing function in $u$. \end {enumerate}\end{proof}

